Surface Reconstruction Using Rotation Systems

Inspired by the seminal result that a graph and an associated rotation system uniquely determine the topology of a closed manifold, we propose a combinatorial method for reconstruction of surfaces from points. Our method constructs a spanning tree and a rotation system. Since the tree is trivially a planar graph, its rotation system determines a genus zero surface with a single face which we proceed to incrementally refine by inserting edges to split faces and thus merging them. In order to raise the genus, special handles are added by inserting edges between different faces and thus merging them. We apply our method to a wide range of input point clouds in order to investigate its effectiveness, and we compare our method to several other surface reconstruction methods. We find that our method offers better control over outlier classification, i.e. which points to include in the reconstructed surface, and also more control over the topology of the reconstructed surface.

==> SigA24/Sections/Method-bak.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\columnwidth]{SigA24/figures/RS.png}
    \caption{$RS$ of an example neighborhood. Taking $v_2$ as an example, it is projected on the disk. Then an angle $\alpha_2$ is calculated as the radian of vertex $v_2$.}
    \label{fig:RS}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\columnwidth]{SigA24/figures/topocheck.png}
    \caption{Topology check for the candidate edge $\left\{u,v\right\}$. \revision{In this example, the candidate edge splits $f_1$ within the right corner. Thus, it passes the topology check.}}
    \label{fig:topocheck}
\end{figure}


\section{Method}
\label{sec:method}
%

\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{SigA24/figures/pipeline.png}
    \caption{Pipeline overview on synthetic letter point clouds. \revision{\sout{General} High-genus} reconstruction follows the bottom pipeline, where $g$ stands for the genus number. Given prior knowledge of genus-0 shape, the shorter pipeline on the top is adapted.}
    \label{fig:pipeline}
\end{figure*}

%
The essence of our algorithm is to construct a tree from the input points and build a triangle mesh from this starting point. A tree is known to be \revision{\sout{a planar graph} genus-0}, and we ensure that \revision{\sout{planarity}it} is maintained while edges are added. As an optional part of the algorithm, handle edges can be added to increase the genus of the reconstructed object. 
%\revision{Before delving into details, it is essential to define two specific types of graph: \textit{genus-0 graph} and \textit{plane projectable graph} (\textit{pp graph}). A genus-0 graph is a graph that can be embedded in manifolds of genus 0. While pp graph is a graph that can be projected along the normal direction as a plane graph.}

In the following, we will discuss all stages in greater detail and we refer the reader to Figure~\ref{fig:pipeline} and Algorithm~\ref{alg:main} for an overview of our pipeline.

\begin{algorithm}
    \caption{\revision{Pseudocode for the main loop}}
    \label{alg:main}
    \revision{
        \KwData{$pts$}
        \KwResult{$M$}
        $org\_pts \gets pts$\;
        $normals \gets \mathrm{estimate\_normal}(pts)$\;
        $proj\_pts, kDTree \gets \mathrm{project}(pts, normals)$\;
        $normals \gets \mathrm{estimate\_normal}(proj\_pts)$\;
        $N \gets \mathrm{find\_components}(kDTree)$\;
        $comp\_id \gets 0$\;
        \While{$comp\_id \leq N - 1$}{
            $G \gets \mathrm{init\_graph}(kDTree, comp\_id)$\;
            $Q \gets \mathrm{sort\_edge}(G)$\;
            $MST \gets \mathrm{init\_MST}(G)$\;
            $\mathrm{build\_RS}(MST, M)$\;
            $edge\_id \gets 0$\;
            \While{$edge\_id \leq Q.\mathrm{size}() - 1$}{
                \If{$\mathrm{topology\_test}(M, Q, edge\_id)$}{
                    \If{$\mathrm{geometry\_test}(M, Q, edge\_id)$}{
                        $\mathrm{insert\_edge}(M)$\;
                    }
                }
            }
            \Comment{Optional: Connect handles, raise genus}
            $\mathrm{connect\_handle}(M)$\;
            $\mathrm{triangulate}(M)$\;
            $\mathrm{export\_obj}(M, org\_pts)$\;
        }
    }
\end{algorithm}
%
\subsection{Initialization}
\label{sec:init}
%
We create the initial graph, \revision{$G=(V, E_G)$}, from the vertex set, $V$. $G$ is a k-nearest neighbor ($k$NN) graph where $k$ is a user\revision{-}defined parameter and the Euclidean distance is used to define the neighborhood. Notably, since the connections are symmetrized for both incident vertices of an edge, a vertex in $G$ may have more than $k$ neighbors.
\revision{Connections are now removed in the cases where connected vertices $u$ and $v$ have normal vectors which point in opposite directions, i.e. $\mathbf N_u \cdot \mathbf N_v < 0$. This consistency test helps us avoid connecting vertices on either side of thin structures.}

Subsequently, the mesh \revision{$M=(V, E_M)$} is initialized to the minimum spanning tree (MST) of $G$. Clearly, both the neighborhood and the minimum spanning tree vary if the point cloud is influenced by noise, and in Section~\ref{sec:projection_dist} we will discuss how this is taken into account.

At this time, \revision{\sout{we also establish}}a rotation system $RS$ \revision{is established for $M$}. \revision{\sout{which} It} determines a cyclic ordering of the neighbors of each vertex. The rotation system is computed based on the normal vector associated with each vertex. While our approach thus relies on vertex normals, the normal computation is not an intrinsic part of the scheme, and our code allows for user-provided normals. In both respects, our approach is similar to many other reconstruction methods.

The construction of the cyclic ordering around an arbitrary vertex, $u$, with neighbors, $v_i$, \revision{where $\left\{u,v_i \right\} \in \sout{E} E_M$} is shown in Figure~\ref{fig:RS}. Each neighboring vertex, $v_i$, is projected into the plane defined by the position $\mathbf{p}_u$ and normal, $\mathbf N_u$, of vertex $u$. We compute the angle of each projected vertex relative to an arbitrary reference direction and thereby obtain a cyclic ordering of the neighbors of $u$ which is finally stored in $RS$.

The significance of the rotation system is that it defines the \revision{\sout{$\rho$ operator} operator $\rho$}. Initially, $M$ is a tree that we can construe as a mesh with a single face that can be traversed starting from an arbitrary halfedge using repeated application of $\tau = \rho \circ \iota$. \revision{In the next phase, additional edges from $E_G$ will be added to $E_M$. As $E_M$ expands, $RS$ will be updated accordingly.} Of course, $M$ does not contain all edges of $G$, and at any time the cyclic ordering is restricted to the subset of halfedges included in $M$.

In addition to the rotation system, we need to be able to keep track of the face associated with each halfedge. A balanced binary tree (not to be confused with the minimum spanning tree of $G$) is used for this purpose. From the tree, the face associated with each halfedge can be retrieved, and we can update the tree efficiently when a new edge is inserted, splitting one of the faces into two faces (for more information, please refer to Section~\ref{sec:Face}). 

%With $RS$ settled, faces introduced in Section~\ref{sec:face_def} can be tracked. In practice, we use a tree structure to store a sequence of halfedges in one face, so that given any halfedge, the corresponding face identifier can be retrieved (for more information, please refer to Section~\ref{sec:Face}). In this way, any edge connection can be detected and categorized into one of the two Euler operators introduced in Section~\ref{sec:euler_op}. The initialization of the tree structure for $M$ is trivial because it is currently an MST, which only contains a single face.

Finally, all edges in $G$ are sorted in the order of increasing length to be examined in the next stage.
%\Andreas{Really are we not just sorting the edges? The difference is slight, but a priority queue only really makes sense if it is updated. On the other hand, the difference in performance is slight, so we can just change the text to say that we sort the edges if it is not updated later?!}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4\columnwidth]{SigA24/figures/planar.png}
%     \caption{An example illustrating the difference between plane graph and planar graph.}
%     \label{fig:plane_and_planar}
% \end{figure}

\subsection{Edge Insertion}
\label{sec:edge_insertion}

In the edge insertion stage, we iteratively insert valid edges from \revision{\sout{$G$} $E_G$ into  \sout{the mesh $M$} $E_M$}, thereby splitting a face of $M$ as illustrated in Figure~\ref{fig:edge_insertion}.
\revision{\sout{The edges are sorted according to length, and an} An} edge is considered valid for $M$ if it passes two tests, the topology test and geometry test, which ensure that $M$ \revision{\sout{remains a valid} remains a genus-0 graph and locally a pp graph. In other words, the first test is required to ensure that we do not make any topological errors and the second test ensures we avoid flipped triangles and overlapping edges in the mesh.} 
\revision{It is important to note that which connections we can make depends on the rotation system which, in turn, is based on the normal vectors. Obviously, the dependency on normal vectors means that the rotation system is sensitive to changes in normal direction. Fortunately, the tests ensure that undesirable connections are avoided, but, in rare cases, isolated vertices are left out because an insufficient number of incident edges can be inserted. In Section~\ref{sec:normal-noise-test} we further investigate the effect of noisy normal vectors on the reconstruction.}

\revision{\sout{Recall that the edges of a genus 0 mesh constitute a {planar} graph.  A graph is planar if it can be embedded in 2D in such a way that no two edges intersect except at vertices. In the following, when we refer to $M$ as being planar, it means that the edges of $M$ form a planar graph. It is also important to distinguish between planar and plane graphs. A plane graph is a graph that is actually embedded in 2D without any edges crossing each other. Hence, a plane graph is necessarily a planar graph, but the converse is not true. }}

\revision{\sout{The first of our two tests, which we \revision{\sout{denote} refer to as} the topology test, ensures that the mesh remains \revision{\sout{planar} genus-0} if the edge candidate is inserted. \revision{\sout{This may seem sufficient, but in some cases, a planar graph can be difficult to embed in 2D despite (in fact) being planar.}However, it doesn't get rid of potential intersections of triangles. For this reason, we also carry out the heuristic geometry test which checks that \sout{edges do not cross locally}it suffices a pp-graph within a defined neighborhood of any vertex.} Both of these tests are described in the following.}}
%
\subsubsection{Topology Test}
\label{sec:topotest}
%
\revision{\sout{The topology test ensures that the entire graph remains planar when a new edge is added.}} First, we check that the endpoints of the candidate edge belong to the same face\revision{\sout{.},} $f$. Next, it is verified that both of the corners which are split when the candidate edge is inserted belong to $f$. \revision{We refer the reader to Section~\ref{sec:face_def} for the definition of corner.} If this test is not passed, we reject the candidate edge.

In order to carry out the topology test in practice, we store the face associated with each halfedge. When a candidate edge $\left\{u,v\right\}$ is considered, we check that all the halfedges before and after $\{u,v\}$ in the rotation system, i.e. $h_1,h_2,h_3$ and $h_4$, are associated with the same face, $f_1$. Please refer to Figure~\ref{fig:topocheck} for an illustration.

\begin{figure}[]
    \centering
    \includegraphics[width=1.0\columnwidth]{SigA24/figures/ab1.png}
    \caption{Example for the necessity of topology test. The left mesh is reconstructed with both tests, while the right one is reconstructed without \revision{the} topology test. A red triangle is formed which result\revision{s} in an undesirable hole.}
    \label{fig:ab1}
\end{figure}

It is clear that $M$ remains \revision{\sout{planar} genus-0} if the edge candidate passes the topology test because $|E|$ and $|F|$ both increase by one. Consequently, the left\revision{-}hand side of the Euler-Poincare formula \eqref{eq:euler} does not change. This also implies that \revision{\sout{the}} the topology test ensures that handles are not inserted at this stage, \revision{\sout{and this is the reason} which is why our method enables reconstruction} with topology control. 

%
\subsubsection{Geometry Test}
%
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\columnwidth]{SigA24/figures/geometry_test.png}
    \caption{Geometry test for edge \{$u,v$\}.\revision{ With a search ball of radius $\frac{1}{2} l + L_{\max}$ and centered at the midpoint of the edge candidate, this test will check if any existing edge associated with vertices inside this search ball intersects with the candidate edge within the tangent plane.}
    }
    \label{fig:geom_test}
\end{figure}

The geometry test ensures that a 2D projection of a local neighborhood of the graph remains a plane graph, i.e. pp-graph, when a new edge is added. As depicted in Figure~\ref{fig:geom_test}, the local neighborhood is defined as a ball with a radius of $\frac{1}{2} l + L_{\max}$, where $l$ is the length of the edge candidate and $L_{\max}$ is the maximum length of any edge in $G$. The plane, $P$, passes through the midpoint of the candidate edge and its normal is defined as the average of the normals at the endpoint vertices.

Any edge for which it is true that either endpoint belongs to the local neighborhood is projected into $P$ and we test for intersection with the candidate edge. If there is an intersection, we reject the candidate edge.

%The geometry test is similar to the test performed by Mencl and Müller\cite{Mencl98}.
We can understand the geometry test as ensuring that $M$ remains a \revision{\sout{plane} pp }graph locally. However, in regions where the normal changes rapidly, this can be insufficient to guarantee that $M$ remains \revision{\sout{a planar graph} genus-0} as shown in Figure~\ref{fig:ab1}. Hence, we need the topology test. In fact, it is important to stress that even if topology control is not desired, the topology test is needed in cases where the tangent plane changes rapidly. In such cases, the geometry test may pass for edges that connect different faces as illustrated in Figure~\ref{fig:ab1}.


\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\columnwidth]{SigA24/figures/ab2.png}
    \caption{Example for the necessity of geometry test. The left mesh is reconstructed with both tests, while the right one is reconstructed without \revision{the} geometry test. The \revision{graph remains genus-0\sout{local graph of the mesh is still planar}}, but not any edge candidate left can pass the corner check of \revision{the} topology test. Thus, a hole is left here and the same reason for any other place of the reconstructed mesh.}
    \label{fig:ab2}
\end{figure}


\revision{\sout{On the other hand, just like the geometry test} Symmetrically}, the topology test is not sufficient in itself. As shown in Figure~\ref{fig:ab2}, there are cases where an edge that passes the topology test would lead to \revision{undesirable configurations, such as intersections, \sout{that are highly undesirable}}but do not \revision{increase the genus number\sout{cause the graph to be non-planar}. \sout{The reason \revision{\sout{for this}}is that a graph can be planar yet very far from being plane.}} Fortunately, these cases are easily dealt with by the geometry test. 

Candidate edges \revision{\sout{which} that} pass both the geometry and topology test can safely be inserted. However, the two tests do not guarantee the quality of the triangles. In order to prevent skinny triangles, i.e. caps or needles with one angle close to $180^\circ$ or $0^\circ$, respectively, we also perform a quality check before insertion. This is discussed in Section~\ref{sec:quality_concern}.

%Summing up, the geometry test ensures that $M$ remains plane (in a local and somewhat loose sense), and the topology test ensures that $M$ remains strictly planar.

\subsection{Handle Connection \& Triangulation}
\label{sec:handle}

Up to this point, $M$ is guaranteed to be of genus-0, i.e. of sphere topology, but some of the faces of $M$ likely consist of many edges. Given such a large face, $f_1$, and a vertex, $v$, that belongs to $f_1$. $v$ may either lack connections to other vertices of $f_1$ because there is a gap in the input point cloud or because the unused edges of $G$ which are incident on $v$ connect it to a different face, $f_2$. In the former case, we would want to leave $f_1$ as a hole, but in the latter case, we may want to insert a handle edge between $f_1$ and $f_2$


% After the insertion of edges, the mesh $M$ reaches a state where the majority of possible connections have been established. However, if the shape is of genus greater than zero some \textit{cracks} will remain. As illustrated in Figure~\ref{fig:pipeline} (lower right), cracks need to be closed to form topological handles,

To merge $f_1$ and $f_2$, we need to close the \textit{cracks}. A crack is constituted by a pair of faces $f_1$ and $f_2$ such that halfedges on one side are associated with $f_1$, while halfedges on the other side are associated with $f_2$. We create a set of handle edges by finding vertices belonging to a face $f_1$ that are connected to a different face and whose corner (i.e. the corner that would be split if the edge were inserted) has an angle greater than $\pi$. For further explanation of the choice of $\pi$, please refer to Section~\ref{sec:quality_concern}. Such handle edges are now inserted if they pass the geometry test described above. The topology test does not apply since it would trivially fail for handles. On the other hand, small, undesired handle candidates are often present locally -- in particular on noisy meshes. \revision{\sout{For this reason} Thus}, we need a different test for handle insertion.
%\Andreas{I think we need to explain why the angle must be greater than $\pi$}

\revision{\sout{In light of the fact that handles represent global structures,} Through extensive experiments, we found handles often represent global structures, which means} the vertices incident on them usually have a short Euclidean distance but are connected by a long shortest path within the graph. Thus, we use a threshold, $n$, on the number of edges in the shortest path between the incident vertices of the handle candidate edge, to cull undesirable handles. A higher value of $n$ corresponds to fewer handles being connected. In our implementation, an effective setting for $n$ is $50$. 

After connecting all handle edges that pass the above test, a final triangulation is performed. At this point, most of the faces are indeed triangles, but since we reject some edges due to quality concerns both during edge insertion and handle insertion (c.f. Section~\ref{sec:quality_concern}), not all faces are fully triangulated. After handle insertion, our face data structure is no longer valid since it can only be efficiently updated when faces are split and not merged. Fortunately, the rotation system is unaffected, and the triangulation only performs ear clipping, i.e. it connects two vertices known to belong to the same face. More details are provided in Section~\ref{sec:add_face}.
%
\subsection{Reconstruction from Noisy Point Clouds}
\label{sec:projection_dist}
%
Scanned point clouds are inherently noisy since scanning is a measurement process. Moreover, several sub-scans are often combined during reconstruction. These may not be perfectly aligned, introducing another source of high-frequency noise.

%Arguably, noise resilience is one of the most important reasons to use volumetric methods over combinatorial methods. 

Noise can be both tangential and normal to the surface. While tangential noise does not affect the reconstruction, normal noise can result in large Euclidean distances between points that are close in the tangent plane. To mitigate this issue, two operations are taken for specified noisy data. 

Firstly, we use the provided/estimated normals to project the points onto the tangent planes and compute the projected distances rather than the Euclidean distances for all distance calculations in the algorithm. To define projection distance, we need some preliminary definition: for edge $e = \{u,v\}$, $e_{//v}$ refers to the projection of $e$ on the tangential plane of $v$. The same applies \revision{\sout{for} to} $u$. The projection distance $|e|_p$ is then defined as
%as Eq. \ref{eq:projection_dist}.
%
\begin{equation}
    \label{eq:projection_dist}
    |e|_p = (|e_{//v}| + |e_{//u}|)/2 \enspace .
\end{equation}
%
However, the kd-tree used for computing the initial graph $G$ is, of course, unaffected by the tangential distances and still based on the Euclidean distance. This can lead to both spurious and missing connections. Therefore, we also project the input points to the average tangent plane of their k-neighborhood and rebuild the kd-tree. Inspired by \cite{Digne2011}, we restore the input points to their original position before the mesh is output. 
% This approach enables the acquisition of a more noise-resilient graph throughout the whole reconstruction procedure. 

It is reasonable to ask why we do not simply compute the Euclidean distance after projecting the points. The reason is that \revision{
%normals are estimated based on the neighborhoods, unevenly distributed vertices are not ensured to be perfectly aligned within a plane. That means
even after the above smoothing, two connected points never lie exactly in each others tangent plane. Hence, there is a meaningful difference between the Euclidean distances and the tangent plane projected distance
} \revision{\sout{the projected points still retain variation along the normal direction}}, and we obtain the best results by using the pure tangent plane distance. 

% \revision{A simplified example is illustrated in Figure~\ref{fig:layers}. Suppose the height difference between two layers is longer than those neighboring connections after projection. In that case, no connections will be made between layers, although they should belong to the same plane before projection.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\columnwidth]{SigA24/figures/layers.jpg}
%     \caption{\revision{It is not guaranteed that the estimated normal of each vertex fits all local planes. When vertices are unevenly distributed, few vertices are sampled around the red vertex, the projection tends to generate two separated layers.}}
%     \label{fig:layers}
% \end{figure}

%One may wonder that: since we project the input points to the tangent plane, why do we need the projecting distance at all? This is related to the nature of scanned noisy data. As our method prefers smooth changed normal along the surface, we tend to estimate normal with a large number of neighbors. However, this leads to the insensitivity of the normal to the local curvature, i.e. high-frequency details in a small area may not be captured by the normal. The Euclidean distance between the projected points may not be equivalent to what we want - a distance on the tangent plane. Thus, We need the direct definition of projection distance to cancel the influence of the noise along the normal direction.

% \Andreas{I think this section needs a quick rewrite since it is unclear what the relationship is between tangent plane distance and smoothing and how smoothing is performed.}
% \Ruiqi{I rewrote and added some details in the last second paragraph, is it clear now? Maybe I didn't get unclear point.}
% \Andreas{The question is this: one might ask why we first compute the symmetrized tangent plane distance since we also project the points onto a smooth surface. A symmetric distance could also be computed from the projected points, but maybe it is better to use the tangent plane distance?}

